Botnets Breaking Transformers: Localization of Power Botnet Attacks Against the Distribution Grid

Traditional botnet attacks leverage large and distributed numbers of compromised internet-connected devices to target and overwhelm other devices with internet packets. With increasing consumer adoption of high-wattage internet-facing "smart devices", a new "power botnet" attack emerges, where such devices are used to target and overwhelm power grid devices with unusual load demand. We introduce a variant of this attack, the power-botnet weardown-attack, which does not intend to cause blackouts or short-term acute instability, but instead forces expensive mechanical components to activate more frequently, necessitating costly replacements / repairs. Specifically, we target the on-load tap-changer (OLTC) transformer, which uses a mechanical switch that responds to change in load demand. In our analysis and simulations, these attacks can halve the lifespan of an OLTC, or in the most extreme cases, reduce it to $2.5\%$ of its original lifespan. Notably, these power botnets are composed of devices not connected to the internal SCADA systems used to control power grids. This represents a new internet-based cyberattack that targets the power grid from the outside. To help the power system to mitigate these types of botnet attacks, we develop attack-localization strategies. We formulate the problem as a supervised machine learning task to locate the source of power botnet attacks. Within a simulated environment, we generate the training and testing dataset to evaluate several machine learning algorithm based localization methods, including SVM, neural network and decision tree. We show that decision-tree based classification successfully identifies power botnet attacks and locates compromised devices with at least $94\%$ improvement of accuracy over a baseline "most-frequent" classifier.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> figures/401_lifespan_vs_ALR_20percent.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=.8\textwidth]{images/401_lifespan_vs_ALR_20percent.png}
  \vspace{-10pt}
  \caption{OLTC lifespan degrading as a function of attacker load ratio (ALR) and attack strategy, focused on the lowest values of ALR, for the flip, heuristic, and random attacks, respectively.}
  \Description[Three lines showing how OLTC lifespan decreases with ALR.]{Three line graphs, with the X axis "ALR" ranging from 0.0 to 0.10, and the Y axis "lifespan" ranging from 1.0 to 0.0. Each of the three lines drop from 1.0 to around 0.20 for ALR values between 0.0 to 0.20.}
  \label{fig:401_lifespan_vs_ALR_20p}
\end{figure} 

==> figures/401_taps_vs_ALR_30percent.tex <==
\begin{figure}[Hh]
  \centering
  \includegraphics[width=.8\textwidth]{images/401_taps_vs_ALR_30percent.png}
  \caption{Number of OLTC tap changes as a result of ALR and attack strategy for low values of ALR, for lower values of ALR, for the flip, heuristic, and random attacks, respectively.}
  \Description[Three lines showing how OLTC taps per day increases with ALR.]{Three line graphs, with the X axis "ALR" ranging from 0.0 to 0.10, and the Y axis "taps" ranging from 0 to 400. Each of the three lines increase from around 35 taps per day, curving upwards. The "rand" method is a bumpy line increasing to about 150 taps per day for ALR 0.10. The "flip" method reaches about 200, while the "aggr" method is slightly higher, reaching about 300.}
  \label{fig:401_taps_vs_ALR_30p}
\end{figure} 

==> figures/fig_power-consumption.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.5\textwidth]{images/powercon.pdf}
  \caption{Power consumption of PowerBot} 
  \Description[Two power consumption graphs, showing the behavior of a air conditioner and water heater activating on-and-off to a "set point" throughout the day.]{Two separate line graphs, one for air conditioner power consumption and another for water heater power consumption. Both have X-axes of "Time" (minutes) from 0 to 1440 minutes. Both have Y-axes of "Power" (kW). The air conditioner graph has a Y axis ranging from 0 to 2 kW, and the water heater graph has a Y axis ranging from 0 to 8 kW. The air conditioner is active from 0 to 200 minutes, in that time taking on a roughly constant value of about 1.5kW. This line falls to near zero (plus some noise) before activating again for a several-minute spike. The air conditioner graph falls to near-zero and rises to about 1.25kW repeatedly throughout the day, with twenty-seven total activations throughout the day. The water heater graph also spikes on-and-off, but the spikes reach about 4.25 kW and is active less, reaching thirteen activations throughout the day.}
  \label{fig:power_consumption}
\end{figure}

==> section_a1_summary.tex <==
\subsection{Attack Problem}

So, we take our IEEE 123 grid, and target OLTC 1 since it seems the easiest. To make things simple, we select these 13 nodes. We consider two dimensions, ``how much influence does the attacker have" and ``which combination of 13 nodes does the attacker have".

We simulate in timesteps of one minute. In each minute, the attacker can turn any number of controlled devices on or off. The attacker gets to read anything about the grid state, and can synchronously control its devices.

We simulate this with OpenDSS and CREST!

The attacker's goal is to maximize the number of tap changes within a 24 hour period (1440 minutes.) The theoretical maximum of simulated tap changes is 1440, a 40x increase from the nominal value of 36 (and so, representing a decrease in OLTC lifespan to only 2.5\%.)

An attacker may wish to operate more discretely and avoid detection, causing a lower rate of tap changes but also delaying countermeasures.



==> section_reinforcement_learning.tex <==
\section{Reinforcement Learning} \label{sec:reinforcement_learning}

\subsection{Problem formulation}
\songyang{Please write down how you formulate your decision making problem such that is can be solved by RL. It includes how many agents there are, what is the state and action for each agent. Do you consider discrete or continuous states? Do you consider discrete or continuous actions? Do you have state transition function? Whether it is deterministic or stochastic? Do you consider stochastic or deterministic policy? What is your policy? What is your objective? Is your state fully observable or partially observable?}

\subsection{Reward function}
\songyang{Define the reward function for the RL agent clearly for your problem}

\subsection{Neural Network Design}
\songyang{Present the neural network structure and explain why you have such a design. If you use Q-learning, then just add Q-network. If you consider actor-critic algorithm, please introduce both actor and critic networks.}

\subsection{Algorithm}
\songyang{Do you have special design for your algorithm? If not, write down the how to adapt classic algorithms into your problem.}

